PBE-CC: Congestion Control via Endpoint-Centric, Physical-Layer Bandwidth Measurements

Wireless networks are becoming ever more sophisticated and overcrowded, imposing the most delay, jitter, and throughput damage to end-to-end network flows in today's internet. We therefore argue for fine-grained mobile endpoint-based wireless measurements to inform a precise congestion control algorithm through a well-defined API to the mobile's wireless physical layer. Our proposed congestion control algorithm is based on Physical-Layer Bandwidth measurements taken at the Endpoint (PBE-CC), and captures the latest 5G New Radio innovations that increase wireless capacity, yet create abrupt rises and falls in available wireless capacity that the PBE-CC sender can react to precisely and very rapidly. We implement a proof-of-concept prototype of the PBE measurement module on software-defined radios and the PBE sender and receiver in C. An extensive performance evaluation compares PBE-CC head to head against the leading cellular-aware and wireless-oblivious congestion control protocols proposed in the research community and in deployment, in mobile and static mobile scenarios, and over busy and quiet networks. Results show 6.3% higher average throughput than BBR, while simultaneously reducing 95th percentile delay by 1.8x.

==> Mot.tex <==
\section{Measurement and Motivation}
The fundamental challenge that congestion control algorithms face when work on cellular networks is the variations of capacity of the wireless cellular link~\cite{Sprout,ABC,Verus}.
We observe that the variations mainly stem from three sources. 
Firstly, the wireless channel quality varies, due to the user mobility or interference from neighbouring cell towers. The channel quality affects the wireless data rate of the cellular link supports. 
Secondly, the competition for limited bandwidth between mobile users that associates with the same cell tower. 
Thirdly, the carrier aggregation. Since the aggregated cells are dynamically activated/de-activated, the maximum bandwidth the cellular network can allocate for one user changes accordingly. 
Furthermore, due to carrier aggregation, an end\hyp{}to\hyp{}end connection is affected by the dynamics of all its aggregated cells. 
The key observation we make in this paper is that, the mobile user can accurately estimate the capacity of the wireless cellular link and track its variations at millisecond granularity using the decoded control messages. 

\subsection{Tracking the Capacity Variations}
\label{s:track_variation}
We demonstrate that the mobile user is able to estimate and track the capacity of wireless cellular link using preliminary experiments. We setup a remote server at Amazon AWS cloud as the sender and use a Samsung S8 as the receiver. 

\begin{figure}[tbh]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{fig/Mot_Rate_PRB.pdf}
        \caption{The wireless physical rate $R_w$ and the allocated PRBs.}
        \label{fig:mcs_phy_rate}
    \end{subfigure}
    
    
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{fig/Mot_Rate_hor.pdf}
        \caption{The received transport layer data rate from the UDP socket.}
        \label{fig:ca}
    \end{subfigure}
    \caption{The mobile experiment. }
    \label{fig:UDP_rate}
\end{figure}


% \begin{figure*}[htb]
%      \begin{minipage}[htb]{0.33\linewidth}
%         \centering
%         \includegraphics[width=0.98\textwidth]{fig/Mot_mcs_phy_rate.pdf}
%         \caption{The wireless physical rate the cellular link supports.}
%         \label{fig:mcs_phy_rate}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[htb]{0.33\linewidth}
%         \includegraphics[width=0.99\textwidth]{fig/Mot_mcs_prb.pdf}
%       \caption{The allocated PRBs for the user.}
%       \label{fig:mcs_PRB}
%     \end{minipage}
%     \hfill
%      \begin{minipage}[htb]{0.33\linewidth}
%         \centering
%         \includegraphics[width=0.98\textwidth]{fig/Mot_mcs_rate.pdf}
%         \caption{The received data rate from the UDP socket.}
%         \label{fig:UDP_rate}
%     \end{minipage}
%     % \vspace{-0.5cm}
% \end{figure*}
\parahead{Tracking the wireless channel variations}
In this experiment, we let the sender sends UDP traffic with a fixed offered load of 12~Mbit/s. We put the mobile phone at a fixed location with \textit{reference signal received power} (RSRP) of -95~dbm and receive for 10 seconds statically. We then move the phone to a new location with RSRP of -108~dbm within 5 seconds. We let the phone receive for another 10 second statically at the new location. In this experiment, the wireless channel quality decreases due to mobility. The cell tower reacts to the channel variation by adjusting its \textit{modulation and coding scheme} (MCS) and notifying the receiver of the adjustment via control message. 
We extract the MCS index and calculate the wireless physical data rate $R_w$ for each subframe, \ie, the number of bits transmitted per PRB, according to Table 7.1.7.2.1 of~\cite{TS213}. 
We plot the $R_w$ in Figure~\ref{fig:mcs_phy_rate}. 
We see that, the wireless physical data rate maintains stable at 1076 bits per PRB for the first 10 seconds, gradually decrease to 800 bits per PRB in the next five seconds, and at last maintain stable at last 10 seconds. 
The variation of the wireless data rate matches with the pattern of the decrease of the wireless channel. 

\parahead{Tracking the bandwidth variations}
The mobile user tracks the number of PRBs that the cell tower allocates by decoding the control messages. 
We plot the number of allocated PRB within each subframe in above experiments in Figure~\ref{fig:mcs_phy_rate}. 
Since the sender is sending with a fixed data rate, the cell has to increase the bandwidth to counteract the effect of decreasing channel quality. 
As a result, we see that the number of PRB increases in the last 10 seconds. 
We further confirm this by plotting the received data from the user's UDP socket in Figure~\ref{fig:UDP_rate}, 
from which, we see that the cellular network maintains a stable delivery rate to the user via jointly adjusting the wireless data rate and allocated bandwidth.
In this experiment, the cell has idle bandwidth so it can maintain the target delivery rate by increasing the bandwidth.


As the wireless frequency bandwidth of one cell is shared by multiple users, idle bandwidth appears when the cell finishes delivering the traffic of any user, which happens frequently.
An responsive congestion control should be able to detect the amount of emerging idle bandwidth and increase its sending rate accordingly.
A legacy mobile user, however, only decodes its own control messages, so by default it cannot track the PRB allocation for other users and thus identify the idle bandwidth.
We observe that the physical control channel is not encrypted, so any legacy mobile user is actually able to decode all the control messages sent over the control channel. 
Prior work on LTE sniffing such as LTEye~\cite{LTEye} and OWL~\cite{OWL}, have demonstrated the feasibility. 
Based on such an observation, we program the mobile user and enable it to decode all the control messages sent over the control channel of the cell.


To demonstrate the detected idle bandwidth, we conduct an experiment in late night, so there is not many active users and the cell has large number of idle bandwidth. 
We let the sender send traffic to one mobile user (a Samsung S8) with fixed load of 30~Mbit/s for 60 seconds. 
We also setup another AWS server, sending traffic to anther mobile user (a Xiaomi MIX3) with a fixed speed for five seconds. 
We repeat the traffic every five seconds, with speeds increasing from 30~Mbit/s to 50~Mbit/s with a step size of 5~Mbit/s.
We plot the number of allocated PRBs (for S8 and for all other mobile users including MIX3) in each subframe in Figure~\ref{fig:idle_bandwidth}. 

\begin{figure}[htp]
\centering
\includegraphics[width=\linewidth]{fig/Mot_idle_band.pdf}
\caption{PRB allocation of every subframe.}
\label{fig:idle_bandwidth}
\end{figure}
We see that when the transmission to MIX3 is stopped, the connection with S8 cannot fully utilize the channel bandwidth of the cell tower, so many PRBs are left idle. 
The S8 can directly detect such idle bandwidth by decoding the control messages, without any probing for bandwidth operations that most end\hyp{}to\hyp{}end congestion control algorithms, including BBR~\cite{BBR}, CUBIC~\cite{CUBIC} and PCC~\cite{PCC,PCC-v}, require. 
We also observe that, when the connection with MIX3 is competing for the shared bandwidth with connection with S8, the bandwidth of the cell is fully utilized by these two connections. 
At last, we observe that the bandwidth are fairly share by two users (around 50\% for both user), no matter how fast the sender sends to MIX3, 
since the cell tower guarantees the fairness between connections that go through it when performs the resource allocation. 

\begin{figure}[htp]
\centering
\includegraphics[width=\linewidth]{fig/Mot_CA_trigger.pdf}
\caption{The process of activation/de-activation of a secondary cell. When the offered load exceeds the maximum capacity of the primary cell, a queue is built up. 
Cellular network activate a secondary cell to support the high data rate of 40~Mbit/s and de-activate the cell when the offered load decreases to 6~Mbit/s.}
\label{fig:CA_trigger}
\end{figure}
\parahead{Tracking the carrier aggregation}
Since every cell sends its control messages via its own control channel\footnote{Even though cross cell scheduling, \ie, sending control messages of one cell via control channel of another cell, is possible according to the standard, we did not observe any service provider implement this functionality.}, we can monitor the activation/de-activation process of the aggregated cells by decoding the control messages of all the cells in the list the cell configures for each user. 
To demonstrate the activation and de-activation of cells, we let the sender send to a receiver (Samsung S8 connecting to a primary cell that has 10~MHz bandwidth and thus has maximum of 50 PBRs) with a fixed offered of 40~Mbits for two seconds and switch to offered load of 6~Mbit/s for one second.
The offered load of 40~Mbit/s exceeds the maximum capacity of the primary cell, so it causes packet buffering at this cell, 
even when all the bandwidth are allocated for this user, as shown in Figure~\ref{fig:CA_trigger}. 
We also see from this figure that, the cellular network detects the packet buffering and activate a secondary cell to help deliver the data to the user, at 0.13 seconds. 
Since 40~Mbit/s is below the aggregated capacity of the primary and secondary cell, so the cellular network drains the built queue within 0.6 seconds. 
The secondary cell is de-activated, \ie, not PRB is allocated to this user from the secondary cell, after the offered load decrease to 6~Mbit/s.


==> bkup.tex <==
\section{Introduction}
We study the TCP congestion control problem in LTE networks. Even though, TCP congestion control for wired internet has been researched for decades, there is a key difference between the wired internet and LTE networks: the last hop of a LTE link is wireless, \textit{i.e.,}  the wireless link between the cell tower and the \textit{user equipment} (UE). The heterogeneity of the link throughput (10s of Gbps for wired network and maximum hundreds of Mbps for LTE wireless link) make the congestion control challenging. 

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{fig/2_case.pdf}
\caption{The available throughput for a LTE TCP link. Specifically, in case one, the wired link provides higher throughput than the wireless link. The throughput bottleneck is the wireless link. In case 2, the wireless link provides high throughput and the bottleneck becomes the wired link.}
\label{fig:2_case}
\end{figure}

The physical data rate of the Ethernet and the wireless link gives the maximum achievable throughput. During transmission, the available throughput of the wired and wireless link is dynamic, as the wired part of the LTE link is shared with many other internet users and the wireless part is shared with all UEs connected to the same cell tower. Therefore, the bottleneck of the LTE link could shift between the wired and wireless links, just as shown in Fig.~\ref{fig:2_case} shows. 

The key challenge of TCP congestion control is to measure the throughput of the bottleneck. In this paper, we need to answer to questions: first, how can we differentiate the two possible cases in Fig.~\ref{fig:2_case}; second, how to measure the throughput of bottleneck in two cases. We want to note that due to the huge gap between the physical data rate that can be supported by Ethernet and LTE wireless link, the bottleneck is the wireless link for most of the cases. 

\section{Detecting the bottleneck}
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{fig/detect_bottleneck.pdf}
\caption{The number of empty or idle resource blocks indicate whether the wireless link is fully utilized or not.}
\label{fig:bottleneck}
\end{figure}

\textbf{Key metric:} the idle or empty physical resource blocks. Idle resource blocks means the wireless link is not fully utilized. If we can fully utilize all resource blocks of the wireless link without significantly increase the delay, then the bottleneck is the wireless link. Otherwise, the bottleneck is the wired link. 


\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/thput_50.png}
\caption{Measured throughput of TCP link with congestion window size 100, 150, 200, 250, 300 and 350.}
\label{fig:thput_50}
\end{figure}
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/delay_50.png}
\caption{Measured delay of TCP link with congestion window size 100, 150, 200, 250, 300 and 350.}
\label{fig:delay_50}
\end{figure}
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/idle_prb_50.jpg}
\caption{Measured idle resource blocks of the LTE wireless link for a TCP link with congestion window size 100, 150, 200, 250, 300 and 350.}
\label{fig:idle_prb_50}
\end{figure}

\subsection{Case one}
In order to verify this, we conduct an experiment measuring the throughput and delay of a LTE TCP link. We also record the number of idle resource blocks of the wireless part of the LTE link. We fix the congestion window for 10 seconds and then change the windows to a larger value. The measured throughput, delay and number of idle resource blocks are plotted in Fig.\ref{fig:thput_50}, Fig.\ref{fig:delay_50} and Fig.\ref{fig:idle_prb_50}. We could see from these figures that:
\begin{itemize}
\item Throughput increases linearly with the congestion window size. The delay doesn't increase with the window size until the wireless channel is almost fully utilized. 
\item Less idle resource blocks are left when the window size increases. 
\item There is no obvious queuing delay when the window size is smaller than 300.
\item The delay is more sensitive to the background traffic when the channel is close to be fully utilized and hence larger variation on the delay is observed. 
\end{itemize}

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/thput_100.png}
\caption{Measured throughput of TCP link with congestion window size 100, 200, 300, 400 and 500.}
\label{fig:thput_100}
\end{figure}
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/delay_100.png}
\caption{Measured delay of TCP link with congestion window size 100, 200, 300, 400 and 500.}
\label{fig:delay_100}
\end{figure}
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/idle_prb_100.jpg}
\caption{Measured idle resource blocks of the LTE wireless link for a TCP link with congestion window size 100, 200, 300, 400 and 500.}
\label{fig:idle_prb_100}
\end{figure}
To see what happens when there are packets buffer at the base station, we conduct another expeirment with the same setup except configuring the congestion window to 100, 200, 300, 400 and 500. The measured throughput, delay and number of idle resource blocks are plotted in Fig.\ref{fig:thput_100}, Fig.\ref{fig:delay_100} and Fig.\ref{fig:idle_prb_100}. We observe that:
\begin{itemize}
\item When the channel is fully utilized, increasing the window size only increases the delay without affecting the throughput.
\item The number of idle resource blocks are almost zero when the channel is fully utilized.
\item Packets are buffered at the based station when the window size is larger than 300.
\end{itemize}

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/bkg_traffic.png}
\caption{(a) the overall throughput of the LTE link; (b) the throughput of the target UE.}
\label{fig:bkg_traffic}
\end{figure}
Finally, we also plot the throughput of the whole LTE link in Fig.\ref{fig:bkg_traffic}(a) and the throughput of the target UE in Fig.\ref{fig:bkg_traffic}(b). We see that the wireless channel reaches its maximum throughput and the UE is also close to the maximum throughput it can obtain. 

\subsection{Case two}
Missing

\section{Congestion control algorithm}
In this section, we introduce the LTE PHY-aware congestion control algorithm. 
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/cc_v1.pdf}
\caption{The architecture of the proposed congestion control system.}
\label{fig:sys_arch}
\end{figure}

\subsection{System architecture}
Our system is built on top of LTEScope. LTEScope provides the MCS index, allocated PRBs and TB error rate of the target UE by decoding the LTE control channel, just as shown in Figure~\ref{fig:sys_arch}. We implement a LTE channel capacity tracker, which estimates the capacity of the UE based on the extracted physical layer parameters. LTEScope is capable of decoding the control message of all active UEs of one cell, so that it also provides the overall bandwidth usage of the cell. We buffer the estimated capacity and cell usage of most recent 128 sub-frames in a circular buffer. 
We maintain a separate buffer for every aggregated cell of the UE. 
The LTE congestion control algorithm takes the buffered data as input, calculates the congestion control feedback (\textit{i.e.}, 1, decreasing or increasing the congestion window, and 2, the speed of the decrease/increase) and sends the feedback via ACK packets to the sender.  


\subsection{Capacity of the LTE TCP link}
The key challenge for TCP congestion control is to measure and track the capacity of the link. 
When the bottleneck is located at the wired sub-link, relying on end-to-end signals such as round-trip time (RTT) to estimate the capacity has been shown to work well. 
We introduce how to estimate the link capacity of LTE wireless sub-link. 

LTE wireless link capacity is determined by three parameters: 1, the modulation, coding rate and spatial streams used by LTE cell tower to transmit data to the UE; 2, the available bandwidth for the UE including the allocated bandwidth to the UE and the idle bandwidth of the cell; 3, the packet loss rate. We decode the control channel to extract these parameters, based on which we estimate the capacity of a single cell. 
When carrier aggregation is triggered for the UE, we estimate the overall LTE capacity by summing up the capacities of all aggregated cells.


\subsection{Slow start} We use similar slow start algorithm as traditional TCP congestion control algorithm such as CUBIC. 
In the beginning of the slow start, the sender approaches the capacity by increasing its sending rate exponentially. Specifically, the sender doubles the congestion window size every RTT. The UE monitors the channel usage and stop the exponential rate increasing if the usage exceeds 90\%. The sender then switch to linearly increase, \textit{i.e.}, increasing the window size by one for every received ACK. The sender stop the increase when the usage achieves 98\%. 

When carrier aggregation is not triggered during the slow start, we will saturate the primary cell for 40~ms instead of stopping at 98\% cell usage, to force the LTE cell tower enabling the carrier aggregation. If carrier aggregation is enabled during the slow start, we stop the exponential increase when the overall usage of all aggregated cell exceed 90\%. 

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig/control.pdf}
\caption{The work flow of congestion control algorithm.}
\label{fig:work_flow}
\end{figure}

\subsection{Congestion control}

We target at fully utilizing the LTE capacity and at the same time without saturating the LTE link. 
Therefore, after the slow start, we aim to maintain a high overall channel usage (larger than 95\% but smaller than 100\%).
We plot the work flow of our congestion control algorithm works in Figure~\ref{fig:work_flow}. 
Based on our target, we calculate the control feedback and send it to the sender via ACK. 
The sender adjust the congestion window size according to the control feedback.
For a specific congestion window, the practical LTE control channel condition can be measured via LTEScope. 
As we have introduced in above section, LTEScope provides the measured channel usage. 
A straightforward way of calculating the control feedback is to calculate gap between the target channel usage with the measured channel usage, based on which we infer whether we should decrease or increase the congestion and the speed of the decrease or increase. 

The cell usage is, however, only a good indicator of link saturation but not a good signal for rate adaptation. 
For example, when a competing traffic appears, the target UE shares the cell bandwidth with the competing UE so that the capacity of the target UE decreases. The overall cell usage, however, maintains high during this process. The correct action that should be taken by target UE is reducing the sending rate, which can be inferred from the available capacity. Another example is that in mobile scenario, the channel capacity may decrease with the decreasing channel quality. Without decreasing the sending rate, the cell usage maintains high but the packets are buffered at the LTE cell tower and introducing excessive delay. All the aforementioned cases can be identified by tracking the UE's channel capacity.

We thus calculate the control feedback using both channel usage and UE's channel capacity. Specifically, we divide the channel usage into two cases, smaller or larger than 95\% and we identify the channel capacity as increasing, decreasing and stable. 
When the channel usage is smaller than 95\%, we always increase the congestion window size. The increasing speed is the same as the slow start, \textit{i.e.}, exponential increasing if smaller than 90\% and then switching to linear increase.
When the channel usage is larger than 95\% and the channel capacity is decreasing, we decrease the congestion window accordingly. 
Specifically, the new congestion window is decreased to $\alpha \cdot cwnd$, where $cwnd$ is the previous congestion window size and $0<\alpha<1$ is a parameter determining the decreasing speed. 
We determine the value of $\alpha$ according the decreasing amount and speed of the UE's capacity. 
At last, we keep the congestion window unchanged when the channel usage is larger than 95\% and the capacity is not decreasing.



% We thus tracks the available channel capacity of the target UE and indicates the sender about the variations of the capacity. The sender increases its rate with the increasing capacity and vice versa. The speed of rate increase depends on the speed and size of the increasing capacity. If we observe that the link is saturated for 50~ms, we will decrease the sending rate until the cell usage decrease to 95\%. 
% The UE monitors the channel usage of the primary cell and indicates the sender when the usage of primary cell achieves 90\%. The sender then increase its sending rate linearly until 98\% channel usage is achieved. 
% During this process, the UE also monitors whether the carrier aggregation is triggered. If CA is triggered, the sender 
% In case one, we need to measure the capacity of the wireless link to adjust the window, since the LTE wireless link is the bottleneck. In case two, we can measure the instantaneous throughput of wireless link as the capacity of the wired link. 

% The capacity of the LTE wireless link is represented as:
% \begin{eqnarray}
% 	\label{eqn:cap}
% 	\mathbf{C}(N_{prb}, M) =  N_{prb} \times T(M),
% \end{eqnarray}
% where $N_{prb}$ is the number of physical resource blocks, $M$ is the MCS index of the transmission and $T(M)$ gives us the number of bits contained in one physical resource block when the MCS index is $M$. If we know the the number of allocated physical resource blocks for one UE, we can calculate its instantaneous throughput based on Eq.\ref{eqn:cap}. If we know both the number of allocated resource blocks for one UE and idle resource blocks of the link, we can calculate the maximum achievable capacity for the specific UE. 

% From Eq.~\ref{eqn:cap}, we see that there are two important parameters that affects the capacity of the LTE wireless for one specific UE, \textit{i.e.,} the number of physical resource blocks $N_{prb}$ and the MCS index $M$. We thus study them in the following sections. 
% \textbf{MCS index} The modulation and coding rate used for transmitting data to a specific UE, is determined by the wireless channel quality. If a UE is in static state, then the wireless channel quality is stable and similar MCS index will be used (MCS is hardly the same as there are 32 different MCS choices). If the UE is mobile, then the channel quality varies and so does the MCS index. 
% \textbf{Physical resource blocks} The allocated resource blocks for the UE and the idle resource blocks varies with the traffic pattern between the cell tower and all active UEs that associated with the cell tower. 

